VC dimensions of group convolutional neural networks

We study the generalization capacity of group convolutional neural networks. We identify precise estimates for the VC dimensions of simple sets of group convolutional neural networks. In particular, we find that for infinite groups and appropriately chosen convolutional kernels, already two-parameter families of convolutional neural networks have an infinite VC dimension, despite being invariant to the action of an infinite group.

==> definitions.tex <==
\raggedbottom
\allowdisplaybreaks[1]
\usepackage{sistyle} % or siunitx
\newcommand\bSI[1]{{\small[\SI{}{#1}]}}

\makeatletter
\newlength\unitwdth
\newlength\numwdth
\settowidth\unitwdth{\bSI{m^3.kg^{-1}.s^{-2}}~}
\settowidth\numwdth{Subsect 99}
\newlength\tdima
\newcommand\SIdescr[2]{%
    \setlength\tdima{\linewidth}%
    \addtolength\tdima{\@totalleftmargin}%
    \addtolength\tdima{-\dimen\@curtab}%
    \addtolength\tdima{-\unitwdth}%
    \addtolength\tdima{-\numwdth}%
    \parbox[t]{\tdima}{%
        #1
        \leaders\hbox{$\m@th\mkern \@dotsep mu\hbox{\tiny.}\mkern \@dotsep mu$}%
        \hfill
        \ifhmode\strut\fi
        \makebox[0pt][l]{%
            \makebox[\unitwdth][l]{}%
            \makebox[\numwdth][r]{#2}}}}
\makeatother

\newcommand{\depth}{L}
\newcommand{\size}{M}
\newcommand{\first}{\operatorname{fi}}
\newcommand{\last}{\operatorname{la}}
\newcommand{\sizefirst}{M_{\operatorname{fi}}} 
\newcommand{\sizelast}{M_{\operatorname{la}}} 
\newcommand{\Parallel}[1]{\mathrm{P}\left(#1\right)} % parallelization
\newcommand{\dParallel}[1]{\mathrm{FP}(#1)}

\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Hil}{\mathcal{H}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Sh}{\mathbb{S}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Rcaltilde}{\widetilde{\mathcal{R}}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\dx}{\, \mathrm{d}x}
\newcommand{\deta}{\, \mathrm{d}\eta}
\newcommand{\Rtwo}{\mathbb{R}^2}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\ftilde}{\widetilde{f}}
\newcommand{\fhat}{\widehat{f}}
\newcommand{\ghat}{\widehat{g}}
\newcommand{\psihat}{\widehat{\psi}}
\newcommand{\thetatilde}{\tilde{\theta}}
\newcommand{\varthetatilde}{\tilde{\vartheta}}
\newcommand{\psitilde}{\tilde{\psi}}
\newcommand{\psitildehat}{\widehat{\widetilde{\psi}}}
\newcommand{\phihat}{\widehat{\phi}}
\newcommand{\Phitilde}{\widetilde{\Phi}}
\newcommand{\ehat}{\widehat{e}}
\newcommand{\xhat}{\widehat{x}}
\newcommand{\yhat}{\widehat{y}}
\newcommand{\psiab}{\psi\left( \frac{t-b}{a} \right)}
\newcommand{\Lone}{L^1(\R)}
\newcommand{\Ltwo}{L^2(\R)}
\newcommand{\epsilontilde}{{\tilde{\epsilon}}}
\newcommand{\epsilonhat}{{\hat{\epsilon}}}

\newcommand{\Short}{\mathcal{S}}
\newcommand{\Wave}{\mathcal{W}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\intR}{\int \limits_\R}
\newcommand{\intRtwo}{\int \limits_{\R^2}}
\newcommand{\summn}{\sum \limits_{m,n\in\Z}}
\newcommand{\summ}{\sum \limits_{m\in\Z}}
\newcommand{\sumn}{\sum \limits_{n\in\Z}}
\newcommand{\sumj}{\sum \limits_{j\in\Z}}
\newcommand{\sumk}{\sum \limits_{k\in\Z}}
\newcommand{\suml}{\sum \limits_{l\in\Z}}
\newcommand{\HRule}{\rule{\linewidth}{0.8mm}}
\newcommand{\ti}{\textit}
\newcommand{\fa}{ \qquad \text{ for all }}
\newcommand{\lb}{\left(}
\newcommand{\Thresh}{\mathbf{Thresh}}
\newcommand{\rb}{\right)}
\newcommand{\NN}{\mathcal{NN}}
\newcommand{\kssupp}{k\text{-sing supp}}
%\newcommand{\log}{\text{log }  }
\newcommand{\eps}{\varepsilon}
\newcommand{\Realization}{\mathrm{R}}
\newcommand{\mult}{\Phi^{Z,d,n,l}_{\mathrm{mult};\tilde{\epsilon}}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

\newcommand{\vect}{\mathbf{vec}}
\newcommand{\Paral}{\mathrm{P}}
\newcommand{\CalO}{\mathcal{O}}
\newcommand{\CalQ}{\mathcal{Q}}
\newcommand{\CalD}{\mathcal{D}}
\newcommand{\CalS}{\mathcal{S}}
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\Schwartz}{\mathcal{S}}
\newcommand{\Fourier}{\mathcal{F}}
\newcommand{\TestFunctionSpace}{C_c^\infty}
\newcommand{\DistributionSpace}{\mathcal{D}'}
%\newcommand{\supp}{\mathrm{supp}}
\DeclareMathOperator*{\supp}{supp}
\newcommand{\DecompSp}{\mathcal{D}}
%\newcommand{\with}{\,\middle|\,}
\newcommand{\with}{\,:\,}
\newcommand{\identity}{\mathbf{Id}}
\DeclareMathOperator{\spn}{span}
\newcommand{\Indicator}{{\mathds{1}}}
\newcommand{\bracket}[1]{{\left\langle #1 \right\rangle}}
\newcommand{\question}[1]{\mybox{gray}{
\textbf{Question:} \textit{#1}}}
\newcommand{\RestrictedNeurons}[2]{\mathfrak{RNN}_{#1} (#2)}

\newcommand{\FirstN}[1]{\{1,\dots,#1\}}

\newcommand{\FiniteScaleProjection}{\tilde{P}^{(J)}_{\mathrm{int}}}


\newcommand{\bfTPs}{\mathbf{T_{\Phi_s}}}
\newcommand{\bfTPw}{\mathbf{T_{\Phi_w}}}
\newcommand{\bfTP}{\mathbf{T_{\Phi}}}

\newcommand{\ciGamma}{\overset{\circ}{\Gamma}}

\newcommand{\brac}[2]{\left( 1+ |#1|^2 \right)^{\frac{#2}{2}}}

\newcommand{\bfTPsA}{\mathbf{T_{\Phi_s}^*}}
\newcommand{\bfTPwA}{\mathbf{T_{\Phi_w}^*}}
\newcommand{\bfTPA}{\mathbf{T_{\Phi}^*}}

\newcommand{\da}{\daleth}%{\textarabic{ﻒ}}
\newcommand{\g}{\gimel}%{\textarabic{ﻎ}}

\newcommand{\phiint}{\phi^{\textintb}}

\newcommand{\conc}{{\raisebox{2pt}{\tiny\newmoon} \,}}
\newcommand{\sconc}{\odot}

\newcommand{\phiright}{\phi^{\textright}}
\newcommand{\cN}{\mathcal{NN}}
\newcommand{\cRN}{\mathcal{RNN}}
\newcommand{\phileft}{\phi^{\textleft}}
\newcommand{\psiint}{\psi^{\textintb}}
\newcommand{\psiright}{\psi^{\textright}}
\newcommand{\psileft}{\psi^{\textleft}}
\DeclareMathOperator{\textintb}{b}
\DeclareMathOperator{\loog}{loog}
\DeclareMathOperator{\Lip}{Lip}
\DeclareMathOperator{\textright}{right}
\DeclareMathOperator{\textleft}{left}
\newcommand{\Ident}{\mathbf{Id}_{\mathbb{R}^{d(\epsilontilde)}}}

\newcommand{\bdWaveS}{\mathcal{W}} %% boundary wavelet system
\newcommand{\bdWaveSDual}{\mathcal{W}^d}
\newcommand{\Lp}[2]{L^{#1}{#2}}
\newcommand{\Hs}[2]{H^{#1}{#2}}

%\def\diag{{\text{\rm diag}}}

\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem*{remark*}{Remark}
\newtheorem*{proposition*}{Proposition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}{Fact}


\DeclareMathOperator{\spann}{span \,}
\DeclareMathOperator{\suppp}{supp \,}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\ran}{ran \,}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand\bigforall{\mbox{\Large $\mathsurround0pt\forall$}}
\newcommand\bigexists{\mbox{\Large $\mathsurround0pt\exists$}}
\DeclareMathOperator{\Exists}{\bigexists}
\DeclareMathOperator{\Forall}{\bigforall}
\DeclareMathOperator*{\interior}{int\,}


\newcommand{\relu}{\mathrm{ReLU}}
\newcommand{\vcdim}{\mathrm{VCdim}}

\newcommand{\ExtOp}{\tilde{E}}
\newcommand{\ExtOpMod}{E}

\newcommand{\ppc}[1]{{\color{blue}[PP: #1 ]\color{black}}}
\newcommand{\pp}[1]{{\color{blue} #1 \color{black}}}
